Diagnosing failures of fairness transfer across distribution shift in real-world medical settings

Diagnosing and mitigating changes in model fairness under distribution shift is an important component of the safe deployment of machine learning in healthcare settings. Importantly, the success of any mitigation strategy strongly depends on the structure of the shift. Despite this, there has been little discussion of how to empirically assess the structure of a distribution shift that one is encountering in practice. In this work, we adopt a causal framing to motivate conditional independence tests as a key tool for characterizing distribution shifts. Using our approach in two medical applications, we show that this knowledge can help diagnose failures of fairness transfer, including cases where real-world shifts are more complex than is often assumed in the literature. Based on these results, we discuss potential remedies at each step of the machine learning pipeline.

==> derm/derm.tex <==
\subsection{Predicting skin conditions in dermatology}
\label{sec:derm}

In this task, we are interested in predicting common skin conditions (26 conditions plus an additional `other' category to capture the long tail), based on one or multiple images of the pathology of interest and additional metadata \citep{Liu2020-qr}. As is relatively common in healthcare settings, the model is trained on source data, and considered for application on target data that has been collected using different protocols in a different clinical environment \citep{Koh2020-cr}. The data used as source is a subset of the data described in \citep{Liu2020-qr}. Briefly, it consists of de-identified retrospective adult cases from a teledermatology service serving 17 sites from 2 states in the United States. Each case contained 1-6 clinical photographs of the affected skin areas as well as patient demographic information and medical history (see Table S1 of \citep{Liu2020-qr}). We split the source data such that it comprises 12,024 cases for training, 1,925 for validation and hyper-parameter tuning and 1,924 for testing. The target data, unobserved at model development time, comes from skin cancer clinics in Australia and New Zealand and was partially labelled, leading to 21,661 cases used for model evaluation. We consider a second target dataset of 1,843 labelled teledermatology cases from Colombia in Sec.\ref{app:derm_target2}.

% \noindent \textbf{Ethics approval:} the images and metadata were de-identified according to Health Insurance Portability and Accountability Act (HIPAA) Safe Harbor prior to transfer to study investigators. The protocol was reviewed by [Anonymous] IRB, which determined that it was exempt from further review under 45 CFR 46.
% Advarra IRB (Columbia, MD)

\subsubsection{Fairness metrics are affected by the environment}
We train a deep learning model to predict skin conditions from the images $X$, age and sex, with an approach similar to \citep{Liu2020-qr,Roy2021-xp}. Based on the source data, we train 10 replicates of the model from different random seeds. Each model is then evaluated based on its top-1 and top-3 accuracy across all conditions on the test set of the source data and on the target data. We assess fairness by estimating the difference in top-k model performance between subgroups. 

\begin{figure*}[!t]
\centering
\includegraphics[width=0.65\linewidth]{derm/Derm_model_performance_unmitigated_top3.png} 
\caption{Model performance in dermatology, as estimated via Top-3 accuracy (in \%). The plot displays the total performance, as well as performance stratified by sex and by age on the source (circles with plain line) and target (diamonds with dashed line) data. Each marker represents one replicate of the model.}
\label{fig:derm_top3}       
\end{figure*}

Overall, our model performs in line with \citep{Liu2020-qr,Roy2021-xp} on the source data
% \footnote{Notice that we are only using a subset of the data, and different splits, leading to an apparent decrease in performance (93\% in \citep{Liu2020-qr} compared to 88\% here).}
, obtaining a top-3 accuracy of $88.52 \pm 0.68 \%$. When stratifying per sex, the model performs slightly better for females ($88.95 \pm 0.93 \%$) than for males ($87.78 \pm 0.52 \%$). We also observe a $1.05\%$ maximum difference across age subgroups, with the 65+ group under-performing ($87.84 \pm 1.70 \%$). We however note that these numbers are close to one another, and that there is no significant difference when considering multiple training seeds. Therefore, not performing any fairness mitigation might seem like a reasonable option.

Nevertheless, the gaps between the groups increase when the environment changes (Fig.\ref{fig:derm_top3}), with the difference between females and males doubling (from 1.17 to 2.33\%) and the maximum age gap reaching 21.32\%. Similar results are obtained when considering top-1 accuracy (Sec.\ref{app:derm_target1_model_perf}). When considering conditions separately, the patterns can vary, but often differ between the source and the target data (Sec.\ref{app:derm_per_cond}). We therefore observe that the fairness metrics are affected by the environment. These results are replicated for the other target dataset considered, leading to similar conclusions.

\subsubsection{A compound shift}
To investigate the nature of the shift, we draw a simplified causal graph of the dermatology task at hand. We consider an anti-causal learning task \cite{scholkopf2012on} $Y \rightarrow X$ to which we add demographics $A$, co-morbidities/medical history $M$ and symptoms $X_s$ and omit unobserved variables (Fig.\ref{fig:derm_shift}(a)).
% , similar in spirit to the anti-causal prediction task discussed in Section \ref{sec:limitations}, but with added metadata. In the source data, we can divide the metadata in multiple variables: demographics $A$, co-morbidities/medical history $M$ and symptoms $X_s$. Each of these plays a different role in the causal graph (see Fig.~\ref{fig:derm_shift}(a)), with the graph itself becoming more complex. We however note that we omit unobservable variables such as environmental factors that could affect the skin or co-morbidities and medical history that are not recorded in the data.

\begin{figure*}[!t]
\centering
%\subfloat[]{
% \scalebox{1}{
% \begin{tikzpicture}
% \node (X) at (1,-1) {$X$};
% \node (A) at (-1.5,-1) {$A$};
% \node (M) at (-1.5,-2) {$M$};
% \node (Y) at (-0.25,-1.5) {$Y$};
% \node (Xs) at (1,-2) {$X_s$};
% \draw[line width=1pt,black, \arr, opacity=0.6](A)--(X);
% \draw[line width=1pt,black, \arr, opacity=0.7](A)--(M);
% \draw[line width=1pt,black, \arr, opacity=0.7](A)--(Y);
% \draw[line width=1pt,black, \arr, opacity=0.7](M)--(Y);
% \draw[line width=1pt,black, \arr, opacity=0.7](Y)--(X);
% \draw[line width=1pt,black, \arr, opacity=0.7](Y)--(Xs);
% \end{tikzpicture}}%}
%\subfloat[]{
\begin{subfigure}[t]{0.03\textwidth}
(a)
\end{subfigure}
\begin{subfigure}[t]{0.45\textwidth}
\resizebox{0.7\linewidth}{!}{
\begin{tikzpicture}[baseline={([yshift={-\ht\strutbox}]current bounding box.north)},outer sep=0pt,inner sep=0pt]
\node (S) at (-0.25,-3) {$S$};
\node (X) at (1,-4) {$X$};
\node (A) at (-1.5,-4) {$A$};
\node (M) at (-1.5,-5) {$M$};
\node (Y) at (-0.25,-4.5) {$Y$};
\node (Xs) at (1,-5) {$X_s$};
\draw[line width=1pt,orange, \arr, opacity=0.6](S)--(Y);
\draw[line width=1pt,blue, \arr, opacity=0.6](S)--(A);
\draw[line width=1pt,green!40!black, \arr, opacity=0.6](S)--(X);
\draw[line width=1pt,blue, \arr, opacity=0.6](S) to [bend right=+78] (M);
\draw[line width=1pt,blue, \arr, opacity=0.6](S) to [bend left=+78] (Xs);
\draw[line width=1pt,black, \arr, opacity=0.6](A)--(X);
\draw[line width=1pt,black, \arr, opacity=0.7](A)--(M);
\draw[line width=1pt,black, \arr, opacity=0.7](A)--(Y);
\draw[line width=1pt,black, \arr, opacity=0.7](M)--(Y);
\draw[line width=1pt,black, \arr, opacity=0.7](Y)--(X);
\draw[line width=1pt,black, \arr, opacity=0.7](Y)--(Xs);
\end{tikzpicture}}%}
\end{subfigure}
\begin{subfigure}[t]{0.03\textwidth}
(b)
\end{subfigure}
\begin{subfigure}[t]{0.45\textwidth}
\includegraphics[width=0.9\linewidth,valign=t]{derm/Derm_demographics_distribution.png} 
\end{subfigure}\\
\begin{subfigure}[t]{0.03\textwidth}
(c)
\end{subfigure}
\begin{subfigure}[t]{0.55\textwidth}
\includegraphics[width=\linewidth,valign=t]{derm/Derm_condition_distribution_elder_female.png}
\end{subfigure}
\begin{subfigure}[t]{0.03\textwidth}
(d)
\end{subfigure}
\begin{subfigure}[t]{0.33\textwidth}
\includegraphics[width=\linewidth,valign=t]{derm/Derm_image_characteristics_distribution_conditioned.png}
\end{subfigure}
\caption{A compound shift in dermatology. (a) Simplified causal structure of the application. $A$ refers to demographic metadata, $M$ to the patient's medical history and comorbidities, $Y$ to the skin condition as labelled by clinicians, $X$ represents the set of pictures of the skin pathology and $X_s$ represents other symptoms as shared by the patient (e.g. whether the lesion is `burning' or `itchy'). In our setup, the environment $S$ directly affects all variables in the graph. (b) Distribution in the source train and in the target dataset of the sensitive attributes, computed in terms of percentage of pre-defined subgroups. (c) Prevalence of each condition in cases where the patients are female and over 65 years of age. (d) Distribution of the number of images in cases labelled as `SK/ISK' in older females. The distributions in the source data are represented on the left, and their corresponding distributions in the target data on their immediate right with a hashed pattern.}
\label{fig:derm_shift}       
\end{figure*}

We first note that the metadata available in the source data is more comprehensive than the data available in the target data, with only age and sex\footnote{Sex is mainly recorded by clinicians, with a small set of the source data containing self-reported sex.} being common to both. These features have different distributions across the two datasets (see Fig.~\ref{fig:derm_shift}(b)), with the population in the source data being typically younger (median age: 40 years old, 25$\%$ quantile: 27, 75$\%$ quantile: 54) than in the target data (median age: 58 years old, 25$\%$ quantile: 44, 75$\%$ quantile: 70). The source distribution also includes more female patients than the target data (62$\%$, compared to 47$\%$). Other demographics and its proxies (e.g. pregnancy status, ethnicity, skin type), as well as $M$ and $X_s$ are absent from the target data. We therefore see direct effects of $S$ on $M, X_s$ and $A$, and add these relationships to the causal graph (Fig.~\ref{fig:derm_shift}a, in purple).

We then assess whether $S$ directly affects the labels. By looking at the graph, we see that a shift on $P(A)$ could lead to a shift on the marginal $P(Y)$. However, conditioning on $A$ and $M$ could lead to an invariance of $Y$ on $S$. As $M$ is absent from the target data, we condition on $A$ only. Using overlap weights to represent the conditioning \citep{Li2019-nv}, we obtain significant differences between $P(Y \,|\, A, S=0)$ and $P(Y \,|\, A, S=1)$ for 24 conditions ($p<0.05$, Bonferroni corrected). Fig.\ref{fig:derm_shift}(c) illustrates the label shift in a specific age and sex subgroup (here females aged 65+, 409 cases in the source, 3,198 in the target data). We see that the source data includes more cases of `eczema' and `psoriasis' and that cancerous conditions such as `basal cell carcinoma' and `melanoma' are more prevalent in the target data. While this analysis is limited due to the absence of $M$ and of sensitive attributes in the target data, our results suggest that the environment also directly affects the labels (orange link in Fig.\ref{fig:derm_shift}(a)). 
% We note that this analysis is limited to the distribution of labels and cannot assess differences in their quality: for instance, the labels for the source data were sourced from multiple clinicians, while some target labels were verified by biopsies. This is an added difference between the two environments (known as annotation shift, \citep{castro2020causality}) that only in-depth dataset knowledge can bring.

% \begin{figure*}[!t]
% \centering
% \begin{subfigure}[t]{0.03\textwidth}
% \textbf{a}
% \end{subfigure}
% \begin{subfigure}[t]{0.4\textwidth}
% \includegraphics[width=0.9\linewidth,valign=t]{derm/Derm_demographics_distribution.png} 
% \end{subfigure}
% \begin{subfigure}[t]{0.03\textwidth}
% \textbf{c}
% \end{subfigure}
% \begin{subfigure}[t]{0.3\textwidth}
% \includegraphics[width=\linewidth,valign=t]{derm/Derm_image_characteristics_distribution_conditioned.png}
% \end{subfigure}\\
% \begin{subfigure}[t]{0.03\textwidth}
% \textbf{b}
% \end{subfigure}
% \begin{subfigure}[t]{0.7\textwidth}
% \includegraphics[width=\linewidth,valign=t]{derm/Derm_condition_distribution_elder_female.png}
% \end{subfigure}
% \caption{A complex shift in dermatology. \textbf{a} Distribution in each dataset of the sensitive attributes, computed in terms of percentage of pre-defined subgroups. \textbf{b} Prevalence of each condition in cases where the patients are female and over 65 years of age. \textbf{c} Distribution of the number of images in cases labelled as `SK/ISK'. The distributions in the source data are represented on the left, and their corresponding distributions in the target data on their immediate right with a hashed pattern.}
% \label{fig:derm_shift}       
% \end{figure*}

Finally, we consider whether the features of the images themselves (designated by $X$) are directly affected by $S$. If the environment does not directly affect the images, then $P(X \,|\, Y, A, S=0)=P(X \,|\, Y, A, S=1)$. However, our weighted t-tests suggest a significant difference between these two distributions ($p<0.05$ on 22 dimensions, corrected). Fig.\ref{fig:derm_shift}(d) illustrates this difference by computing the number of images per case in the group of older females considered above with cases labelled as `SK/ISK' ( source median: 3, $n=61$, target median: 2, $n=341$). This result suggests the existence of the direct path $S \rightarrow X$ and we add this relationship to the graph (green link in Fig.\ref{fig:derm_shift}(a)).

Based on these different analyses, we conclude that the environment is affecting all the nodes in our simplified causal graph, which contrasts with previous works investigating the transferability of fairness. Similar results are obtained for the second target dataset considered, although 17 conditions present invariances to $S$ after controlling for demographics (Sec.\ref{app:derm_target2}). Interestingly, considering only those 17 conditions leads to a noticeable reduction in fairness metric disparities between environments (Sec.\ref{app:derm_target2_model_perf}).

% \subsubsection{Current mitigation techniques for fairness violations under distribution shift are not applicable}
% As we observed, the shift is complex and does not satisfy the assumptions in \citep{Singh2021-og}, or the independence between $A$ and $S$ required for \citep{Schumann2019-nu}. In this case, the meta-learning strategy proposed in \citep{Slack2020-zz} cannot be directly applied as this is a single multiclass problem which does not refer to multiple tasks. In the present case, we also notice that (fairness) mitigation strategies for multiclass applications are scarce \citep[e.g. ][]{Yang2020-nu,Denis2021-of}.

% In addition, the features are pixels and non-semantic, meaning that feature selection techniques that directly test for invariances based on the features are not applicable \citep{Magliacane2018-oh,Singh2021-og}. On the other hand, masking has been used previously to constrain the learning towards specific areas of the image \citep{Ross2017-br,Simpson2019-zh}. In this case, each training image is accompanied by a segmentation of the lesion. By `zooming in' on the lesion, we hope that the model will more easily isolate the signal of interest compared to confounding factors, without discarding (too much) useful signal. While this technique has shown some promise with chest x-rays \citep{Viviano2019-ij}, it is impractical due to the additional requirement of a mask for all training images. In addition, it increases the ratio of signal of interest compared to undesirable signal, but does not exclude such signals. Therefore, in cases where the undesirable signal remains strong in the masked area, the technique comes with no guarantee.

==> ehr/ehr.tex <==
\subsection{Clinical risk prediction from Electronic Health Records}
\label{sec:ehr}
In this application, we predict the clinical outcomes of patients based on EHRs. EHRs record the time series of interactions between a patient and the clinical system (e.g. medication, labs, vitals,~\dots). In the context of EHR data, evidence has previously shown heterogeneity across centers \citep{Wilson2021-uq}. However, important shifts can also be observed within a single system \citep{Nestor2019-dp}. As an example, over half of hospitals in the US with intensive care units (ICUs) only have a single unit where all critically ill patients (medical, surgical, cardiac,~\dots) are admitted \citep{noauthor_undated-ki}. Risk scores, such as the Acute Physiology and Chronic Health Evaluation II (APACHE II) score are used to evaluate all critically ill patients, but do not perform equally across clinical subgroups, e.g. underperforming on patients with cardiac disease~\citep{Pierpont1999-qb}. We illustrate this shift by considering a model developed on data from generalist ICUs and deployed on data from specialized ICUs. The dataset used in this study is the open access, de-identified Medical Information Mart for Intensive Care III (MIMIC-III) dataset \citep{Johnson2016-eu}, which consists of data from admissions to ICUs at the Beth Israel Deaconess Medical Center between 2001 and 2012. Based on clinical input, we consider the Medical ICU (MICU), Surgical ICU (SICU) and Trauma Surgical ICU (TSICU) to be generalist ICUs; whereas the Cardiac Surgery Recovery Unit (CSRU) and Coronary Care Unit (CCU) are specialized ICUs. This split leads to 17,641 patients included in the source dataset and 10,442 patients in the target dataset after cohort selection. Our goal is to predict prolonged ICU stay (i.e. length of stay $>3$ days, as in \citep{Wang2019-ac,Pfohl2021-xn}) using data from the first 24 hours of first ICU admission. Please see Supplement~\ref{app:ehr_data} for additional information.

\subsubsection{Fairness metrics are affected by the shift}
As performed in \citep{Roy2021-rr, Tomasev2019-tu, Tomasev2021-uf}, each patient's medical history is converted to a time series of one-hour aggregates including the different structured data elements (medication, labs, vitals, \dots) represented by numerical and binary variables. Based on the first 24 hourly aggregates, we predict the binary label for prolonged length of stay using a recurrent network architecture \citep{Tomasev2019-tu, Tomasev2021-uf}. We then estimate model performance in terms of accuracy across patients and per sex and age subgroups. In addition to per-group metrics, we compute demographic parity and equalized odds.

Figure~\ref{fig:ehr_acc}(a) displays model accuracy across subgroups on the source and target data. On the source data, the model performs to $78.6 \pm 0.7 \%$ accuracy, with $\sim1\%$ performance gap between sex groups (Female: $77.8 \pm 0.8\%$, Male: $79.2 \pm 0.5\%$), and a gap of $7.4\%$ between age subgroups (18-29: $84.0 \pm 1.6\%$, 30-44: $82.8 \pm 0.9\%$, 45-64: $78.8 \pm 0.5\%$, 65+: $76.6 \pm 0.7\%$). Performance increases slightly between the two environments, with the model reaching $79.7 \pm 0.9\%$. The gap between sexes increases to $2.7\%$ on the target data (Female: $78.0 \pm 0.6\%$, Male: $80.7 \pm 0.5\%$). For ages, the maximum gap remains similar (7\% on average across seeds, 18-29: $82.5 \pm 0.9\%$, 30-44: $84.2 \pm 0.9\%$, 45-64: $83.2 \pm 0.6\%$, 65+: $77.2 \pm 0.6\%$).

\begin{figure*}[!t]
\centering
\begin{subfigure}[!t]{0.03\textwidth}
(a)
\end{subfigure}
\begin{subfigure}[!t]{0.7\textwidth}
\includegraphics[width=\linewidth,valign=t]{ehr/EHR_model_performance_unmitigated_acc.png}
\end{subfigure} \\
\begin{subfigure}[!t]{0.03\textwidth}
(b)
\end{subfigure}
\begin{subfigure}[!t]{0.7\textwidth}
\includegraphics[width=\linewidth,valign=t]{ehr/EHR_model_performance_mitigated_acc.png} 
\end{subfigure}
\caption{Model performance in EHR, as estimated via accuracy. The plot displays the total performance, as well as performance stratified by sex and by age on the source (circles with plain line) and target (diamonds with dashed line) data. Each marker represents one replicate of the model. (a) Un-mitigated. (b) After mitigating for equalized odds across age groups on the source data.}
\label{fig:ehr_acc}       
\end{figure*}

In terms of fairness metrics, demographic parity is $0.002 \pm 0.002$ for sex on the source, and $0.016 \pm 0.003$ on the target. It is $0.05 \pm 0.006$ for age on the source, and $0.066 \pm 0.010$ on the target. For both attributes, we hence observe an increase in demographic parity between the source and the target. Equalized odds do not display a significant difference between the two environments, for age or sex. On the other hand, we observe significant differences in model accuracy for specific subgroups (e.g. 45-64 years old) between the two environments, suggesting that investigating the predictions for specific subgroups is needed, in addition to computing overall scores like demographic parity, equalized odds or maximum performance gaps.

\subsubsection{A compound shift}
We frame this task by referring to the causal graph described in \citep{Singh2021-og}. In their work, the authors used a restricted set of variables related to demographics $A$, comorbidities $M$, observed features $X$ and the label $Y$. Similarly, we define the demographics $A$ as age and self-reported sex, comorbidities $M$ as previous medical history defined by ICD-9 codes \citep{Charlson1987-xb,Deyo1992-ct,Halfon2002-nq,Li2008-go}, observed features $X$ as all labs and vitals, and $Y$ as our prolonged length of stay label. Given that a more comprehensive feature set leads to better predictive performance \citep{Roy2021-rr}, we use all 59,351 features at our disposal and add `treatments' $T$ (e.g. medications) to the graph (Figure~\ref{fig:ehr_shift}(a)). In our graph, $S$ represents the ICU unit type that a patient is admitted to and is therefore correlated with the `reason for the ICU visit' $R$. We note that variables like labs and vitals might correlate with $R$ but that the model does not have a direct access to $R$ within the first 24 hours of admission for which the predictions are issued.

As performed in Section \ref{sec:derm}, we investigate potential (conditional) independencies between the environment and the different variables. We first estimate the distribution of age and sex in each dataset (Figure~\ref{fig:ehr_shift}(b)). We observe that the population in the source is typically younger (median: 62 years old, 25\% quantile: 49, 75\% quantile: 76) than the population in the target (median: 68 years old, 25\% quantile: 58, 75\% quantile: 77, t-test: $p<0.0001$). In addition, the proportion of males in the source and target differ (source: 50\%, target: 65\%). Therefore, $A \nind S$.

\begin{figure*}[!t]
\centering
\begin{subfigure}[t]{0.03\textwidth}
(a)
\end{subfigure}
\begin{subfigure}[t]{0.4\textwidth}
\resizebox{0.65\linewidth}{!}{
\begin{tikzpicture}[baseline={([yshift={-\ht\strutbox}]current bounding box.north)},outer sep=0pt,inner sep=0pt]
\node (S) at (0.25,-0.5) {$S$};
\node (X) at (1,-2) {$X$};
\node (A) at (1,-1) {$A$};
\node (M) at (2,-1.5) {$M$};
\node (Y) at (0,-1.5) {$Y$};
\node (T) at (0,-2) {$T$};
\draw[line width=1pt,orange, \arr, opacity=0.6](S)--(Y);
\draw[line width=1pt,blue, \arr, opacity=0.6](S)--(A);
\draw[line width=1pt,green!40!black, \arr, opacity=0.6](S)to (X);
\draw[line width=1pt,blue, \arr, opacity=0.6](S) to [bend left=+78] (M);
\draw[line width=1pt,blue, \arr, opacity=0.6](S) to [bend right=+78] (T);
\draw[line width=1pt,black, \arr, opacity=0.6](A)--(X);
\draw[line width=1pt,black, \arr, opacity=0.7](A)--(M);
\draw[line width=1pt,black, \arr, opacity=0.7](A)--(Y);
\draw[line width=1pt,black, \arr, opacity=0.7](M)--(Y);
\draw[line width=1pt,black, \arr, opacity=0.7](M)--(X);
\draw[line width=1pt,black, \arr, opacity=0.6](M) to [bend left=+58] (T);
\draw[line width=1pt,black, \arr, opacity=0.7](T)--(X);
\draw[line width=1pt,black, \arr, opacity=0.7](T)--(Y);
\end{tikzpicture}}%}
\end{subfigure}
\begin{subfigure}[t]{0.03\textwidth}
(b)
\end{subfigure}
\begin{subfigure}[t]{0.5\textwidth}
\includegraphics[width=0.9\linewidth,valign=t]{ehr/mimic_demographics_distribution.png} 
\end{subfigure}\\
\begin{subfigure}[t]{0.03\textwidth}
(c)
\end{subfigure}
\begin{subfigure}[t]{0.65\textwidth}
\includegraphics[width=\linewidth,valign=t]{ehr/Mimic_comorbidities-Gender-M-Ages-65-100.png}
\end{subfigure}
\begin{subfigure}[t]{0.03\textwidth}
(d)
\end{subfigure}
\begin{subfigure}[t]{0.25\textwidth}
\includegraphics[width=0.85\linewidth,valign=t]{ehr/label-prevalence-M-65-90-solid_tumor-Vasopressors-Inotropes.png}
\end{subfigure}
\caption{A compound shift in EHR. (a) Causal graph for this application (see text for variable description). (b) Distribution in each dataset of the sensitive attributes, computed in terms of percentage of pre-defined subgroups. (c) Prevalence of comorbidities for male patients over 65 years of age. (d) Prevalence of the label for male patients over 65 with a solid tumor comorbidity and under vasopressors/inotropes. The distributions in the source data (train split) are represented on the left, and their corresponding distributions in the target data on their immediate right with a hashed pattern.}
\label{fig:ehr_shift}       
\end{figure*}

To assess comorbidities, we refer to Elixhauser and Vanwalraven scores for comorbidities \citep{Elixhauser1998-ra, Van_Walraven2009-ei} and compute the scores on the source and target data \citep{Johnson2018-zj}\footnote{Code publicly available at \url{https://doi.org/10.5281/zenodo.821872}}. Figure~\ref{fig:ehr_shift}(c) displays the distribution of comorbities in a specific slice of the data (here older males, $n=3,951$ in source and $n=3,588$ in target). As expected, patients in the target data have a higher prevalence of comorbidities related to the peripheral vascular system than in the source data and $M \nind S \,|\, A$ for 8 comorbidities (weighted t-test: $p<0.05$, Bonferroni corrected).

We repeat the analysis to assess the direct effect of $S$ on the treatments ($P(T \,|\, A, M, S=0) = P(T \,|\, A, M, S=1): p<0.0001$), on the labs and vitals ($P(X \,|\, A, M, T, S=0) = P(X \,|\, A, M, T, S=1): p<0.05$) and on the label ($P(Y | A, M, T, S=0) = P(Y \,|\, A, M, T, S=1): p<0.05$) in Supplement~\ref{app:ehr_shift}. Figure~\ref{fig:ehr_shift}(d) displays the prevalence of prolonged length of stay for the specific subgroup of older males with a history of a solid tumor comorbidity and receiving vasopressors/inotropes ($n=55$ in source and $n=16$ in target). Our results suggest that the shift is compound, i.e. the ICU unit a patient is admitted to will directly affect all variables in our causal graph. We note that this conclusion is not surprising clinically, given that the environment $S$ is correlated with the reason for their ICU admission $R$, and that this reason for admission (unobserved) is a main driver for all variables.


\subsubsection{Fairness properties after mitigation do not transfer}
As the gap between age groups in the source is considerable, we perform post-processing of the predictions to enforce either demographic parity or equalized odds across age subgroups. We use the method in \citet{alabdulmohsin2021}, fitting the debiasing model on the tune split of the source, and applying it to the test set of the source and to the target set.

This results in demographic parity to decrease to value $10^{-5}$ in the source, but to (slightly) increase to value $0.078 \pm 0.025$ in the target data. Similarly, equalized odds decrease to value $10^{-5}$ and the gap in model accuracy between groups is reduced from 7\% to 0.8\% (Figure~\ref{fig:ehr_acc}(b)) in the source, but increases from $0.05 \pm 0.008$ to $0.16 \pm 0.04$ on the target data, and the gap between age groups increases to 11.4\%.
% \begin{figure*}[!t]
% \centering
% \includegraphics[width=0.8\linewidth]{ehr/EHR_model_performance_mitigated_acc.png} 
% \caption{Model performance in EHR as estimated via accuracy after mitigating for equalized odds on the source data. The plot displays the total performance, as well as performance stratified by sex and by age on the source (circles with plain line) and target (diamonds with dashed line) data. Each marker represents one replicate of the model.}
% \label{fig:ehr_mitigated_eo}       
% \end{figure*}

We therefore observe that mitigating for either demographic parity or equalized odds on the source leads to no improvement, or even worsening of the fairness properties on the target. Noteworthy, the variance across seeds also increases on the target, which might highlight a manifestation of underspecification \citep{DAmour2020-bz}.

% \subsubsection{Current mitigation for fairness violations under distribution shift are not applicable}
% \citet{Singh2021-og} clearly mention which shifts can be accounted for by their feature selection strategy: shifts that are mediated by $A$ (i.e. $S \rightarrow A \rightarrow X^d$), or shifts that affect variables $X$ correlated with the outcome $Y$. For the latter, affected variables are considered as `unstable' and need to be removed from the input feature set. In the present case, the graph is more complex, as is the shift, and the covariate shift assumption is not valid (i.e. here $Y \,|\, A, M, T \nind S$). Therefore, the method would lead to an empty feature set. We also note that shifts affecting single variables in $X$ are unlikely due to the presence of correlations among variables (e.g. labs sampled as part of `panels' and not in isolation).
% In terms of experimentally-driven techniques, we observe the same limitation as for dermatology, whereby we only have a single task and the work of \citet{Slack2020-zz} is not directly applicable. Engineering-wise, it is also unclear how provable transfer techniques could apply to the recurrent, multidimensional, sparse problem that represents EHR modeling.


==> technical_limitations.tex <==
\section{Technical and Practical Limitations}
In this section, we review how various transferable fairness approaches that have been proposed in the literature interact with various causal structures of domain shift.
In addition to remarking on particular approaches, we also apply the analysis method of \citet{Singh2021-og} and compute the ``separating set'' of variables that should be included in a model to obtain the worst-case optimal predictor with transferable fairness.
This provides a fundamental baseline for what can be achieved without further restrictions on the problem.
Notably, under many shifts, including compound shifts, this separating set is empty.

